BLISS: Interplanetary Exploration with Swarms of Low-Cost Spacecraft

Leveraging advancements in micro-scale technology, we propose a fleet of autonomous, low-cost, small solar sails for interplanetary exploration. The Berkeley Low-cost Interplanetary Solar Sail (BLISS) project aims to utilize small-scale technologies to create a fleet of tiny interplanetary femto-spacecraft for rapid, low-cost exploration of the inner solar system. This paper describes the hardware required to build a nearly 10 g spacecraft using a 1 m$^2$ solar sail steered by micro-electromechanical systems (MEMS) inchworm actuators. The trajectory control to a NEO, here 101955 Bennu, is detailed along with the low-level actuation control of the solar sail and the specifications of proposed onboard communication and computation. Two other applications are also shortly considered: sample return from dozens of Jupiter-family comets and interstellar comet rendezvous and imaging. The paper concludes by discussing the fundamental scaling limits and future directions for steerable autonomous miniature solar sails with onboard custom computers and sensors.

==> 06_sched.tex <==
\section{Schedule and Future Work}
\subsection{Testing on Earth}
\label{sec:schedule}

Testing on Earth will be accomplished using two test set ups. 
The first will utilize an in-house built 3-axis, 6 DoF force and torque sensing stand capable of measuring the moment of inertia, mass distribution, and dynamic response in orientation and direction of the BLISS spacecraft due to the MEMS GCA motor output. 
The second will be accomplished with the use of the NASA Ames MicroGravity Test Facilty, employing parabolic flight patterns to observe the dynamic responses of the BLISS spacecraft in a microgravity environment. 
\subsection{Testing on Orbit}
\cite{morrow2001solar}

\subsection{First interplanetary mission}
\subsection{Sample Return and Reentry}
\subsection{System re-design}

% \fi
